How Does Batch Normalization Help Optimization?

Batch Normalization (BatchNorm) is a widely adopted technique that enables faster and more stable training of deep neural networks (DNNs). Despite its pervasiveness, the exact reasons for BatchNorm's effectiveness are still poorly understood. The popular belief is that this effectiveness stems from controlling the change of the layers' input distributions during training to reduce the so-called "internal covariate shift". In this work, we demonstrate that such distributional stability of layer inputs has little to do with the success of BatchNorm. Instead, we uncover a more fundamental impact of BatchNorm on the training process: it makes the optimization landscape significantly smoother. This smoothness induces a more predictive and stable behavior of the gradients, allowing for faster training.

==> proofs/output-sensitivity.tex <==
\todo{Do we still want this?}


==> rr.tex <==
\section{Does Internal Covariate Shift Adversely Affect Network Optimization?}
\label{app:rr}
At this point, the claim that there exists a direct link between BatchNorm's performance and either preserving distributional stability or reducing ICS, broadly construed, seems hard to justify. Taking a step back though, it is worthwhile to understand whether ICS is even the right goal in the first place. Interestingly, while \cite{BNpaper} proposed a mechanism to reduce ICS, it did not provide any evidence of the connection between ICS and network optimization.

To address this issue, by proposing an approach that does reduce ICS, as defined in Section \ref{sec:ics}, and examining its effect on training performance. Our approach, \emph{adjusted gradient descent}, corresponds to training the network by updating the layers in a {\em sequential} fashion (from input layer to output layer) instead of the usual, simultaneous fashion. That is, in each training step, instead of computing the gradients for all the layers at once and then applying the corresponding update, we compute the layer gradients and apply the update one by one\footnote{Note that the training time is increased by a factor equal to the depth of the network in this case.}. Observe that by doing so we eliminate the change in gradient direction for a particular layer due to updates to the previous layers, as desired. 

Figure~\ref{fig:rr}(b) compares the training performance of a VGG network with and without correction for ICS, i.e., when we use adjusted gradient descent method and the standard gradient descent method. We observe that even for relatively small learning rates, training with adjusted gradient descent diverges. To understand this finding better, we compare the difference in the training behavior of the two optimization algorithms for a small number of steps. Initially, the loss minimized using the adjusted gradient descent method undergoes a steep decline due to correction for covariate shift. It, however, soon experiences sharp spikes.

This effect turns out to be caused by adjusted gradient descent leading the network towards sharp local minima, which are abundant in the highly non-linear VGG network. 

Indeed, similar effects can be observed when we employ standard training with reduced learning rates (scaled down by the total number of layers in the network). Further, as expected, these effects are not prominent in the \emph{linear} DLN model. However, even in this simplified setting the performance improvement over standard training (due to correcting for covariate shift using adjusted gradient descent) is negligible. 

These observations bring into question the commonly-held belief that ICS is detrimental to network training.
In particular, it appears that training without correcting for ICS could allow the optimization to escape sharp local minima.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[scale=0.34]{Figures/vgg_rr.pdf}
        \caption{}
    \end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[scale=0.34]{Figures/dln_rr}
    \caption{}
\end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.34\textwidth}
        \centering
        \includegraphics[scale=0.34]{Figures/vgg_cs_zoom}
        \caption{}
    \end{subfigure}
    \caption{Training networks with adjusted gradient descent to correct for internal covariate shift: (a) VGG (b) DLN. This suggests that reducing covariate shift is not particularly beneficial for optimization. Note especially the case of the non-linear VGG network, where adjusted gradient descent diverges even at low learning rates. This happens because adjusted gradient descent leads the network to sharp local minima. (Similar effects occur during standard training with low learning rates.)}
    \label{fig:rr}
    \vspace{-0.2in}
\end{figure}


